A 0.2 solar mass protostar with a Keplerian disk in the very young L1527 IRS system

In their earliest stages, protostars accrete mass from their surrounding envelopes through circumstellar disks. Until now, the smallest observed protostar/envelope mass ratio was ~2.1. The protostar L1527 IRS is thought to be in the earliest stages of star formation. Its envelope contains ~1 solar mass of material within a ~0.05 pc radius, and earlier observations suggested the presence of an edge-on disk. Here we report observations of dust continuum emission and 13CO (J=2-1) line emission from the disk around L1527, from which we determine a protostellar mass of M = 0.19 +/- 0.04 solar masses and a protostar/envelope mass ratio of ~0.2. We conclude that most of the luminosity is generated through the accretion process, with an accretion rate of ~6.6 x 10^-7 solar masses per year. If it has been accreting at that rate through much of its life, its age is ~300,000 yr, though theory suggests larger accretion rates earlier, so it may be younger. The presence of a rotationally--supported disk is confirmed and significantly more mass may be added to its planet-forming region as well as the protostar itself.

==> abstract.tex <==
We present high-resolution sub/millimeter interferometric 
imaging of the Class 0 protostar L1527 IRS (IRAS 04368+2557) at $\lambda$ = 870 \micron, 1.3 mm, and
3.4 mm from the Submillimeter Array (SMA) and Combined Array for Research
in Millimeter Astronomy (CARMA). These observations enable us to clearly detect the presence 
of a compact, flattened source (180 AU diameter) in the center of the envelope.
We interpret this object to be an edge-on protostellar disk, consistent with previous observations 
of the apparent disk in L\arcmin-band scattered light. Observations of the $^{13}$CO ($J=2\rightarrow1$) 
transition has enabled us to detect a rotation signature in the disk and constrain the protostellar
mass to be 0.1 $M_{\sun}$, the first ever for such a young protostellar system.
The disk mass is estimated to be 0.029 and 0.009 $M_{\sun}$ from
the 3.4 mm and 870 \micron\ data respectively, assuming isothermal and 
optically thin emission. The millimeter
spectral index is also found to be quite shallow, $\alpha$ $\sim$ 2, implying 
a dust opacity spectral index $\beta$ $\sim$ 0. We model the emission from the disk using Monte Carlo
radiative transfer codes, finding the disk radius to be R = 125 - 150 AU,
highly flared ($H$ $\propto$ $R^{1.3}$), a radial density profile 
$\rho$ $\propto$ $R^{-2.5}$ - $R^{-3}$, and a mass between 0.0075 - 0.01 $M_{\sun}$.
The scale height at 100 AU is 40 AU and is consistent with vertical hydrostatic equilibrium. 
The resolved millimeter observations indicate that disks may
grow rapidly throughout the Class 0 phase and are already quite large by the transition to Class I.
On the whole the mass and radius of the young disk around L1527 is quite similar 
to disks around pre-main sequence stars; however, the disk is considerably more 
vertically extended due to a combination of lower protostellar mass, in addition to infall onto
the disk upper layers.



